Real-Time Edge Intelligence in the Making: A Collaborative Learning Framework via Federated Meta-Learning

Many IoT applications at the network edge demand intelligent decisions in a real-time manner. The edge device alone, however, often cannot achieve real-time edge intelligence due to its constrained computing resources and limited local data. To tackle these challenges, we propose a platform-aided collaborative learning framework where a model is first trained across a set of source edge nodes by a federated meta-learning approach, and then it is rapidly adapted to learn a new task at the target edge node, using a few samples only. Further, we investigate the convergence of the proposed federated meta-learning algorithm under mild conditions on node similarity and the adaptation performance at the target edge. To combat against the vulnerability of meta-learning algorithms to possible adversarial attacks, we further propose a robust version of the federated meta-learning algorithm based on distributionally robust optimization, and establish its convergence under mild conditions. Experiments on different datasets demonstrate the effectiveness of the proposed Federated Meta-Learning based framework.

==> math_def.tex <==
%math operators
%\newcommand{\argmin}{\mathop{\mbox{\rm arg\,min}}}
%\newcommand{\argmax}{\mathop{\mbox{\rm arg\,max}}}
\newcommand{\AR}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mar}[2]{\begin{array}[t]{#1} #2 \end{array}}
\newcommand{\nn}{\nonumber \\}

%math symbol shorforms
\def\pl{(L)}
\def\sg{\sigma}
\def\Sg{\Sigma}
\def\dt{\delta}
\def\Dlt{\Delta}
\def\lb{\lambda}
\def\ep{\epsilon}
%modified on March 15, 2000
\def \scriptf{{{\cal F} }}
\def \tn{\tilde{n}}
\def \b{\beta}
\def \n2{{N_0 \over 2}}
\def \g{\gamma}
\def \G{\Gamma}
\def \et{\eta_{s1}}
\def \ett{\eta_{s2}}
\def \bt{\bar{T}}
\def\ra{\rightarrow}
\def\lra{\longrightarrow}
\def\Lra{\Longrightarrow}
\def\st{\stackrel{a.s.}{\longrightarrow}}
\def\asst{\stackrel{a.s.}{\Longrightarrow}}
\def\pdst{\stackrel{P}{\Longrightarrow}}
\def\ard{\stackrel{(d)}{\longrightarrow}}
\def\pst{\stackrel{P}{\longrightarrow}}
\def\pist{\stackrel{\Pi}{\longrightarrow}}
\def\pitost{\stackrel{\Pi_2}{\longrightarrow}}
\def\dst{\stackrel{{\cal D}}{\Longrightarrow}}
\def\eqa{\stackrel{(a)}{=}}
\def\eqb{\stackrel{(b)}{=}}
\def\eqc{\stackrel{(c)}{=}}
\def\eqd{\stackrel{d}{=}}
\def\leqa{\stackrel{(a)}{\leq}}
\def\leqb{\stackrel{(b)}{\leq}}
\def\leqc{\stackrel{(c)}{\leq}}
\def\leqd{\stackrel{(d)}{\leq}}

\def\Re{\mbox{\rm Re}}
\def\Im{\mbox{\rm Im}}
\def\mmse{\mbox{\scriptsize\textrm{mmse}}}
\def\MMSE{\mbox{\textrm{MMSE}}}
\def\ms{\mbox{\scriptsize \textrm{ms}}}

\def \mb{\mathbf}

\def\kK{\mbox{$k=1, \cdots, K$}}
\def\nN{\mbox{$n=1, \cdots, N$}}
\def\mM{\mbox{$m=1, \cdots, M$}}
\def\lL{\mbox{$l=1, \cdots, L$}}
\def \h5{\hspace{0.5in}}
\def \lf{ L \ra \infty}
\def \nf{ N \ra \infty}
\def \bs{\mbox{\boldmath $s$}}
\def \bS{\mbox{\boldmath $S$}}
\def \bA{\mbox{\boldmath $A$}}
\def \ba{\mbox{\boldmath $a$}}
\def \bB{\mbox{\boldmath $B$}}
\def \bb{\mbox{\boldmath $b$}}
\def \bn{\mbox{\boldmath $n$}}
\def \bC{\mbox{\boldmath $C$}}
\def \bT{\mbox{\boldmath $T$}}
\def \bE{\mbox{\boldmath $E$}}
\def \bG{\mbox{\boldmath $G$}}
\def \bH{\mbox{\boldmath $H$}}
\def \bgamma{\mbox{\boldmath $\gamma$}}
\def \bD{\mbox{\boldmath $D$}}
\def \bd{\mbox{\boldmath $d$}}
\def \bds{\mbox{\scriptsize\boldmath $d$}}
\def \bR{\mbox{\boldmath $R$}}
\def \br{\mbox{\boldmath $r$}}
\def \bv{\mbox{\boldmath $v$}}
\def \bI{\mbox{\boldmath $I$}}

%\def \bIc{\mbox{\boldmath ${\mathcal I}$}}
\def \bLambda{\mbox{\boldmath $\Lambda$}}
\def \bPsi{\mbox{\boldmath $\Psi$}}
\def \bXi{\mbox{\boldmath $\Xi$}}

\def \bM{\mbox{\boldmath $M$}}
\def \bS{\mbox{\boldmath $S$}}
\def \bU{\mbox{\boldmath $U$}}
\def \bV{\mbox{\boldmath $V$}}
\def \bw{\mbox{\boldmath $w$}}
\def \bW{\mbox{\boldmath $W$}}
\def \bZ{\mbox{\boldmath $Z$}}
\def \bzr{\mbox{\boldmath $0$}}
\def \bone{\mbox{\boldmath $1$}}

\newcommand{\mf}{\mbox{\scriptsize\textrm{mf}}}
\newcommand{\eff}{\mbox{\scriptsize \textrm{eff}}}
\newcommand{\SIR}{\mbox{\rm SIR}}
\newcommand{\SINR}{\mbox{\rm SINR}}
\newcommand{\MSIR}{\mbox{\rm MSIR}}
\newcommand{\II}{\mbox{\scriptsize{\rm II}}}
\newcommand{\SNR}{\mbox{\rm SNR}}
\newcommand{\var}{\mbox{\rm var}}
\newcommand{\bigo}{\mbox{\rm O}}
\newcommand{\littleo}{\mbox{\rm o}}
\newcommand{\mrc}{\mbox{\scriptsize\textrm {mrc}}}
\newcommand{\MAI}{\mbox{\scriptsize\textrm {MAI}}}
\newcommand{\egc}{\mbox{\scriptsize\textrm {egc}}}
\newcommand{\slc}{\mbox{\scriptsize\textrm {sc}}}
\newcommand{\gmdist}{\mbox{\rm Gamma}}

